MagicPose: Realistic Human Poses and Facial Expressions Retargeting with Identity-aware Diffusion

In this work, we propose MagicPose, a diffusion-based model for 2D human pose and facial expression retargeting. Specifically, given a reference image, we aim to generate a person's new images by controlling the poses and facial expressions while keeping the identity unchanged. To this end, we propose a two-stage training strategy to disentangle human motions and appearance (e.g., facial expressions, skin tone and dressing), consisting of (1) the pre-training of an appearance-control block and (2) learning appearance-disentangled pose control. Our novel design enables robust appearance control over generated human images, including body, facial attributes, and even background. By leveraging the prior knowledge of image diffusion models, MagicPose generalizes well to unseen human identities and complex poses without the need for additional fine-tuning. Moreover, the proposed model is easy to use and can be considered as a plug-in module/extension to Stable Diffusion. The code is available at: https://github.com/Boese0601/MagicDance

==> sec/cfg.tex <==
\textbf{Image-CFG}
Thanks for the reviewer's kind remind, we'll add a reference to Classifier-Free Guidance ~\cite{ho2022classifier} in the final version. It proposes to train a conditional and an unconditional diffusion model. Then the resulting conditional and unconditional score estimates are combined to attain a trade-off between sample quality and diversity similar to that obtained using classifier guidance. This technique has been widely adopted in diffusion models~\cite{zhang2023adding,rombach2022high,wang2023disco,karras2023dreampose,cao2023masactrl}. Similarly, we also adopt classifier-free guidance for MagicPose. In our case, the conditional score is obtained with both the reference image and pose map as input while only the pose map is fed into the model for the unconditional score estimation. 

From Figure. 5 in our paper, we highlight the effectiveness of each module by \textbf{removing} it from the pipeline (wo stand for without). It's true that Image-CFG is a critical module in our pipeline, but without Image-CFG we can still observe the general shape of the human subject (e.g. the second row) and a less noisy background, compared to removing the appearance control pretraining with our proposed Multi-Source Self-Attention Module. Moreover, Table 3. demonstrates the performance gain of each module in our pipeline. The proposed appearance control pretraining and Disentangled Control with Multi-Source Self-Attention Module boosts the FID from \textbf{288.64} to \textbf{25.50} and Face-Cos from \textbf{0.038} to \textbf{0.426}, while Image-CFG boosts the FID from \textbf{61.33} to \textbf{25.50} and Face-Cos from \textbf{0.272} to \textbf{0.426}.
So we conclude that Image-CFG is an important module for MaicPose, (considering cfg is widely used in diffusion models~\cite{zhang2023adding,rombach2022high,wang2023disco,karras2023dreampose,cao2023masactrl}), but our proposed modules significantly contribute more to the generation quality. 

\textbf{Table 4}
As mentioned in our paper, the purpose of our experiments on Everybody Dance Now~\cite{chan2019everybody} is to demonstrate the generalization ability of MagicPose to in-the-wild motion, e.g. full-body pose, pose from the back and side of the human. So we use the test set of this dataset after training MagicPose on TikTok~\cite{Jafarian_2021_CVPR_TikTok} dataset. It's hard to find the same setting from other works since they use Everybody Dance Now~\cite{chan2019everybody} training set as training data and test set for testing. Here, we use the officially released model weight from DisCo~\cite{wang2023disco}(the most important diffusion model baseline we compared to on TikTok~\cite{Jafarian_2021_CVPR_TikTok} ) and test the method on Everybody Dance Now~\cite{chan2019everybody} test set. The result is shown in Table.~\ref{tab:edn_disco}. We can see that MagicPose provides better generalization ability to in-the-wild motions even with less training data.

\begin{table*}[t!]\vspace{-5pt}
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=1pt}
\caption{Quantitative comparison of the generalization ability of MagicPose and DisCo~\cite{wang2023disco} on Everybody Dance Now~\cite{chan2019everybody} test set. MagicPose has been trained on TikTok~\cite{Jafarian_2021_CVPR_TikTok} only, while DisCo has been trained on TikTok and other datasets~\cite{fu2022stylegan,ge2019deepfashion2,schuhmann2021laion,lin2014microsoft} 
}
\label{tab:edn_disco}
\scalebox{0.8}
{\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}[2]{*}{Method}  & \multicolumn{2}{c}{\textbf{Subject1}} & \multicolumn{2}{c}{\textbf{Subject2}}& \multicolumn{2}{c}{\textbf{Subject3}}& \multicolumn{2}{c}{\textbf{Subject4}}& \multicolumn{2}{c}{\textbf{Subject5}} & \multicolumn{2}{c}{\textbf{Average}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
 & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$  & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$ & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$ & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$ & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$ & \textbf{FID}\ $\downarrow$  & \textbf{PSNR}\ $\uparrow$\\
\midrule
Disco~\cite{wang2023disco}  & 27.98&28.46 & 30.80 & 29.41& \textbf{33.86} & 27.64& 38.77& 28.19& 34.89 & \textbf{28.49}&  33.26 & 28.44\\


 
MagicPose  & \textbf{22.59}  & \textbf{30.67} & \textbf{22.21}  & \textbf{30.13 }  &35.43 &\textbf{29.35}& \textbf{31.72}  & \textbf{29.53}  & \textbf{31.24 }&28.48 & \textbf{28.64 }& \textbf{29.63} \\

\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table*}

==> sec/masactrl.tex <==
Both MasaCtrl~\cite{cao2023masactrl} and Reference Only ControlNet~\cite{Zhang} are inference-only models and require text as appearance guidance input. 
MagicPose is a pipeline that can be fine-tuned on customized data and provide consistent identity-preserving generation without any text prompt.

\textbf{MasaCtrl} also utilizes parallel UNet architecture, however, there are several major differences between MasaCtrl and MagicPose 
\begin{enumerate}
    \item The self-attention key-value pairs from the reference branch in MasaCtrl \textbf{replace} those in SD-UNet, while MagicPose's \textbf{Multi-Source} Self-Attention Module concatenates the key-value pairs from both SD-UNet and appearance control model. 
    \item The replacement of key-value pairs only exists in \textbf{decoder} after specific denoising timestep $S$ and after specific layer index $L$ in MasaCtrl, while MagicPose manipulates all self-attention layers in the encoder, middle block, and the decoder. For both inference and training, the manipulation always exists regardless of timesteps. This ensures our model learns both \textbf{encoding} appearance from the reference image (encoder) and \textbf{generating} identity-preserving results(decoder) from customized data.
    \item Text is required as input to generate an extraction \textbf{mask} for key-value pairs in MasaCtrl, while MagicPose doesn't need any additional text information so that appearance information \textbf{only} comes from the reference image. This further helps our model to strictly preserve the identity and make our approach suitable for the motion retargeting (usually there's no text prompt for this task, since pose map defines the human motion and reference image controls human appearance and background).
\end{enumerate}

\textbf{Reference Only ControlNet} does not have a parallel UNet architecture like the original ControlNet~\cite{zhang2023adding}. Reference Only ControlNet shares the same architecture and weight as SD-UNet and first takes a noisy reference image as the only input. During the denoising process of the reference image, the query key and value from the self-attention layers are saved temporarily in a \textbf{\textit{cache}}. Then the text is fed as input to the SD-UNet again and the denoising process yields image generation output, while the self-attention layers take query key value from the \textbf{\textit{cache}}. In contrast, MagicPose introduces a \textbf{trainable} parallel UNet architecture without text input and the appearance control model implicitly learns how to provide identity control for SD-UNet with Multi-Sourse Self-Attnetion Module during fine-tuning.

==> sec/new_tiktok_table.tex <==
\begin{table*}[t!]
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=1pt}
\caption{Quantitative comparisons of MagicPose with the recent SOTA methods DreamPose~\cite{karras2023dreampose} and Disco~\cite{wang2023disco}. 
% ``CFG'' and ``HAP'' denote classifier-free guidance and human attribute pretraining, respectively. 
$\downarrow$ indicates that the lower the better, and vice versa. Methods with $*$ directly use the target image as the input, including more information compared to the OpenPose~\cite{8765346,simon2017hand,cao2017realtime,wei2016cpm}. $^\dagger$ represents that Disco~\cite{wang2023disco} is pre-trained on other datasets~\cite{fu2022stylegan,ge2019deepfashion2,schuhmann2021laion,lin2014microsoft} more than our proposed MagicPose, which uses only 335 video sequences in the TikTok~\cite{Jafarian_2021_CVPR_TikTok} dataset for pretraning and fine-tuning. \textbf{Face-Cos} represents the cosine similarity of the extracted feature by AdaFace~\cite{kim2022adaface} of face area between generation and ground truth image.
}
\label{tab:quant_comp_tiktok}
{\begin{tabular}{lccccccc}
\toprule
\multirow{2}[2]{*}{Method}  & \multicolumn{6}{c}{\textbf{Image}} & \multicolumn{1}{c}{\textbf{Video}} \\ \cmidrule(lr){2-7} \cmidrule(lr){8-8}
 & \textbf{FID}\ $\downarrow$  & \textbf{SSIM}\ $\uparrow$ & \textbf{PSNR}\ $\uparrow$ & \textbf{LPIPS}\ $\downarrow$ & \textbf{L1} $\downarrow$\ & \textbf{Face-Cos}\ $\uparrow$ & \textbf{FID-VID}\  $\downarrow$ \\
\midrule
FOMM$^*$~\citep{siarohin2019first}  &85.03  &0.648  &29.01  & 0.335  &3.61E-04  &0.190 &90.09 \\
MRAA$^*$~\citep{siarohin2021motion}  &54.47  &0.672  & 29.39  &0.296  &3.21E-04  & 0.337 &66.36 \\
TPS$^*$~\citep{zhao2022thin}  &53.78  &0.673  & 29.18  &0.299  &3.23E-04  &0.280 &72.55  \\
DreamPose~\citep{karras2023dreampose} &72.62    &0.511  &28.11  &0.442 &6.88E-04 & 0.085&78.77  \\ 
DisCo~\cite{wang2023disco} & 50.68    &0.648  &28.81  &0.309  &4.27E-04  & - &69.68  \\
DisCo$^\dagger$~\cite{wang2023disco} &30.75    &0.668  &29.03  &\textbf{0.292}  &3.78E-04  & 0.166 &59.90  \\ 


\midrule

MagicPose  &\textbf{25.50}   &\textbf{0.752 } &\textbf{29.53}  & \textbf{0.292}  &\textbf{0.81E-04} & \textbf{0.426}
 &\textbf{46.30}  \\
\bottomrule
\end{tabular}}
\vspace{-5pt}

\end{table*}

==> sec/rebuttal.tex <==


\input{sec/user_study_table}


% \vspace{-3mm}
\textbf{Participants}
We use \textbf{Prolific}, an online platform designed to connect researchers with participants for academic studies and market research for all our user studies. The participants are English-speaking random users verified by this platform without prior knowledge of computer vision.

\textbf{Criteria for Judgment}
Since our paper focuses on the motion retargeting task, the criteria for evaluation are 1) The appearance (Face, Clothes on the body, Background) of the generation should strictly match the given reference image input. 2) The motions and facial expressions of the generation should strictly match the given pose condition map input. As mentioned in Section A of our Supplementary Material, We ask the participants to choose \textbf{the only one} method which preserves the best identity information for each video subject. 
In order to compare in a professional manner, all the methods are anonymized as A, B, C, D, E, and the order of the generated image from the corresponding method is randomized in each subject comparison, e.g. For comparison of video subject 1, A,B,C,D,E correspond to MRAA, FOMO, TPS, Disco, MagicPose. For comparison of video subject 2, A,B,C,D,E correspond to Disco, MRAA, MagicPose, FOMO, TPS. 


\textbf{Additional Larger-Scale Study}
In order to make the conclusion from our user study statistically significant, we recruited another 60 participants (100 participants in total) from Prolific and extended the user study to a larger scale. The result is presented in Table.~\ref{tab:user_study_rebuttal} and we can still conclude that MagicPose preserves the identity the best compared to prior works.

\textbf{Statistical Analysis}
We perform a chi-square test on our results. For each vote by an participant, we label the chosen method as 1 and the rest methods as 0. Results of such a test are shown in Table.~\ref{tab:user_study_rebuttal}, we compare five methods (A, B, C, D, E) on eight video subjects with the following steps:
\begin{enumerate}
    \item State the \textit{Null Hypothesis}: There is no association between the video subjects and the choice of method. The distribution of votes for each method is the same across all groups, meaning any observed differences are due to chance.

    \item Compute chi-square statistic and p-value: Chi-square statistic: \(116.02\). p-value: \(1.11 \times 10^{-12}\). Degrees of freedom: \(28\).

    \item Conclusion and Discussion: Given the extremely small p-value (much less than 0.05), we can reject the Null Hypothesis. This indicates that there is a statistically significant association between the video subjects and the choice of method. In simpler terms, the differences in vote distribution for the methods across the eight groups are unlikely to have occurred by chance, pointing towards a significant preference pattern among the groups. We conclude that the participants indeed prefer our proposed MagicPose more than other methods.
\end{enumerate}



